Metrical Tagging in the Wild: Building and Annotating Poetry Corpora with Rhythmic Features

A prerequisite for the computational study of literature is the availability of properly digitized texts, ideally with reliable meta-data and ground-truth annotation. Poetry corpora do exist for a number of languages, but larger collections lack consistency and are encoded in various standards, while annotated corpora are typically constrained to a particular genre and/or were designed for the analysis of certain linguistic features (like rhyme). In this work, we provide large poetry corpora for English and German, and annotate prosodic features in smaller corpora to train corpus driven neural models that enable robust large scale analysis. We show that BiLSTM-CRF models with syllable embeddings outperform a CRF baseline and different BERT-based approaches. In a multi-task setup, particular beneficial task relations illustrate the inter-dependence of poetic features. A model learns foot boundaries better when jointly predicting syllable stress, aesthetic emotions and verse measures benefit from each other, and we find that caesuras are quite dependent on syntax and also integral to shaping the overall measure of the line.

==> 011_rhythmmeter.tex <==
\section{Background: Prosody of Poetry}

The discourse on meter, rhythm and prosody in poetry tends to be contentious, and not always clear in its terminology. In this paper, we work with a fairly pragmatic notion of these terms, mixing a linguistic-systematic approach with a historically-intentional one. This entails that we aim at a linguistic description of the features of poetic texts, but also use labels that are borrowed from historically grown traditions to describe certain forms or pattern, without adhering to a particular theory.

The most salient unit of a poem is the verse. Versification then refers to the making of verse or verse craft. Derived from the Lat. \textit{versificatio},
a form combining \textit{versus} (turning a plow at the ends of
successive furrows, which, by analogy, suggest lines of
writing) and \textit{facio} (make), versification for a long time meant making lines. 
With the advent of mod. *free verse, esp. of *composition by open
field, the original sense of versification as making lines
according to some *measure, or *meter (Gr. metron , Old. E.
mete) has expanded to include all aspects of making poetry,
from the smallest aspects of *sound to *stanzas to
whole-poem forms and genres.

Meter is the *measure of sound patterning in verse,
occurring when a rhythm is repeated throughout a
passage of lang. with such regularity that a base unit
(such as a foot) becomes a norm and governs poetic
composition. 

Meter is an idealized pattern, a cultural
construct understood as artistic shaping of the sound
pattern of a lang. All langs. possess the makings of
metrical systems. Metrical verse works the basic properties
of a given lang. to a more highly regularized
level. 

The rhythm of a linguistic utterance is basically the sequence of syllable-related accent values (associated with pitch, duration and volume/loudness values) resulting from the 'natural' pronunciation of a sentence or text by a competent speaker who takes into account the learned inherent word accents as well as syntax- and discourse-driven accents. All acquired top-down knowledge of lexicon, syntax, and prosody of the whole language goes into this pronunciation, but not any particular meter construct. In this 
%particularly relevant latter 
sense, rhythm is driven bottom-up by the wording of sentences. 

In particular uses of language (proverbs, slogans, poems, songs), the rhythm is over-regulated in the direction of a genuine meter. In silent reading of poems, a meter expectation based on acquired knowledge is usually already triggered by the visual perception of a strophic structure. 

%Moreover, German (or English) readers know from experience, for example, that where there is an end rhyme, there is also a meter. (Rhyme is, at least in German, a para-metrical phenomenon. Conversely, there is also meter without rhyme). 

When listening, the perception of an artificially (over)regulated meter is also and especially bottom-up in a relatively short time. Once a meter has been developed (be it top-down and visually, be it bottom-up in the process of silent reading or listening), it is built into the expectation, and it thus acquires the status of a top-down construct that guides (further) reading (on revocation).
Basically, therefore, a meter is primarily, though by no means exclusively and always, an artificial top down construct. Rhythm, on the other hand, is more bottom-up and arises all by itself from 'natural' prosody. 

Further, from about 1550 to at least 1900, most Western
metrical theories derived from *classical prosody, as
that was reinterpreted in successive eras– particularly
in the 18th c., which saw the rise of cl. philology in
Germany. Common to all these theories was the presumption
that, in metrical lines, syllables are to be
taken together in groups, as metrical units; such units
occupy a position in the theory midway between the
metrical position (or syllable) and the line. 
Reformulation of Gr. concepts like the \textit{iamb} 

%Both the
%concept of the metrical foot itself and the particular
%names and forms of the feet were taken directly from
%Gr., all of them being redefined as the accentual equivalents
%of the identical patterns in the quantitative prosody
%of cl. Gr. Th us, the Gr. *iamb, short + long ($u$ –),
%was reformulated as unstressed + stressed (x /). Th e Gr.
%notion of the metron in certain meters was ignored (as
%were, by and large, other cl. concepts such as the colon,
%the *anceps syllable, and * brevis in longo ). 



%Many prosodists
%continued to talk of longs and shorts—indeed, for
%centuries—but, in fact, stress and/or syllable count was
%the basis for most Western meters by about the 4th c.
%ce . Whether the foot was an element of poetic composition
%or merely of analysis—i.e., *scansion—remained
%an issue of dispute.

Line: Self-contained, (rhythmically) bound
Meter: sequence of stress values
Foot:
Caesura:
Main Accents:
Rhythm:
Measure:

Meter signals *genre, elicits the pleasures
of musicality in expectation and surprise, imitates
meaning in the content (see iconicity, mimesis ),
contributes to *tone (e.g., ironic, satiric, oracular, conversational),
and bears social and cultural meanings.
Th e fi rst three of these functions were much studied
by *New Criticism and *structuralism (essays in Sebeok
and in Chatman and Levin). Th e last two of these
functions have been most neglected despite their
analytic potential with respect to critical and cultural
studies (Hurley). Because the defi nitions and limits
of meters are preferences of a group or a time, what is
called a meter can change, and the theories and functions
of meter will also change over time.

ACCENT In Eng., accent is the auditory prominence
perceived in one syllable as compared with others in
its vicinity. Accent and stress are often treated as synonymous,
though some literary scholars and linguists
distinguish the two terms according to a variety of
criteria. Disagreements persist about the source and
acoustical nature of syllabic prominence—loudness,
volume, *pitch, *duration, or some combination of
factors—but they are arguably of peripheral relevance
to the understanding of accent within Eng. poetics.
Th e phenomena of accent vary among langs. and
the poetics associated with them.

II. Rhythm versus Meter . Th e distinction between
rhythm and meter is old, dating to at least the th c.
bce . Th e disagreement between the * metrici and the
rhythmici in ancient Greece refl ected two approaches
to verse, one strictly quantitative, the other musical,
and the two terms have retained these connotations.
Meter is that aspect of regular rhythm that can be labeled
and counted. It is sometimes conceptualized as
an abstract pattern coexisting with the actual, varied
rhythm of the poem’s lang., and most systems of *scansion
are designed to provide a graphic representation of
this pattern, though there is no psychological evidence
for the simultaneous perception of two diff erent levels
in our apprehension of metrical verse. Th e evidence of
Ren. attempts to write vernacular verse in cl. meters,
however, suggests that the intellectual apprehension of
complex metrical patterns can coexist with the aural
appreciation of rhythm (see also classical meters in
modern languages).
When the rhythm-bearing features of a lang. are arranged
in such a way as to produce marked regularity,
and thus the perception of beats, the basis for metrical
organization exists. And when the series of beats and
intervening off beats are themselves organized into patterns,
a meter is perceived, usually in conformity with
a set of numerical constraints that has developed in the
linguistic trad. in question. Meter can thus be understood
as a particular form of rhythm, but it must be
remembered that even the strictest metrical verse will
retain some of the variety and unpredictability of the
language’s native rhythm. Th e establishment of a metrical
pattern will also have an eff ect on the perception
of rhythm, for instance, in the *promotion or *demotion
of certain syllables. Any

\iffalse

VERSIFICATION. Versifi cation refers to the making
of verse or verse craft. Derived from the Lat. versifi catio,
a form combining versus (turning a plow at the ends of
successive furrows, which, by analogy, suggest lines of
writing; see boustrophedon ) and facio (make), versifi -
cation for a long time meant making lines. With the advent
of mod. *free verse, esp. of *composition by open
fi eld, the original sense of versifi cation as making lines
according to some *measure, or *meter (Gr. metron , OE
mete ) has expanded to include all aspects of making poetry,
from the smallest aspects of *sound to *stanzas to
whole-poem forms and genres.
Versifi cation is still sometimes defi ned and used as
synonymous with *prosody (Gr. prosodia , the song accompaniment
to words, pitch variation as spoken; Lat .,
prosodia , the marking of accent on a syllable). Prosody
has referred to the sound patterns of lang. since the
early Ren. and with verse practice since the mid-Ren.
( OED ). With the Ren., experiments with Romance
models spurred close attention to rules for making lines
and stanzas. By the late Ren., when poetry followed the
taste for strict versions of metrical conformity, prosodie
referred to both the practice of marking accents and
to the rules for duration in pronunciation ( OED ). Th e
marking of accents in making meters was a primary and
necessary part of making verse, so the two terms served
equally in discussing verse and became confl ated. To
the present, the two terms are sometimes interchangeable.
W. K. Wimsatt (in ), e.g., was still using versifi
cation to mean the craft of making metrical poetry,
even while John Hollander (in ) was distinguishing
verse, as metered lines, from a mod. sense of poetry, as
requiring the making of new metaphors.

With energetic Ren. experiments in adapting
duration-based cl., It., and Fr. forms to the pitch-based
prosody of Eng. (see classical meters in modern
languages ), versifi cation was often a matter both of
counting syllables and, in some cases, of determining
their lengths as either “short” or “long”; thus, a
versifi er was largely occupied with prosodic considerations.
Med. and Ren. grammars regarded prosody
as pronunciation and often placed verse within the
province of prosody. Because verse was an oral as well
as a written art, pronunciation was a central concern.
With the expansion of styles and forms over the past
century, individual poets and critics may use versifi cation
to refer to various aspects of poetry, incl. rhetorical
structure (see rhetoric and poetry ), point of view,
*fi guration, *diction, *syntax, fi xed forms (such as the
*sonnet), and the use of a particular lyric *genre or
mode (such as *ode, *elegy, dramatic monologue), as
well as sound patterning (e.g., *rhythm, *meter, *assonance,
*consonance, *rhyme), visual patterning (see
visual poetry ), or the blending of the auditory and
the visual, as in the case of *line or stanza integrity.

Th e historical emergence of free verse, along with the
expanded construing of poetry to signify many kinds of
linguistic poesis, has largely rendered versifi cation outmoded
as a term in its original sense.
Contributing to the declining value and signifi cance
of the term versifi cation are the ongoing reconsiderations
of some of the basic terms associated with the
craft of verse. Th e traditional metered line came under
attack during *modernism, when a wave of experimentation
with verse broke the consistency of meters, loosened
them, or attempted to defi ne and use new measures.
Unlike Ren. innovations, modernism exploited
the prosodic potentials in the lang. medium; the importation
of foreign-lang. forms accounted for but a
small portion of new line and verse forms (e.g., from
OE and ME, Japanese, and Chinese). Th e line as it had
been conceived until  was exploded, freeing it to
be redefi ned as metrical, nonmetrical, visual, or newly
defi ned, as in W. C. Williams’s poetry. Th e breakdown
of the traditional meters, with the *prose poem and
*concrete poetry being the extreme forms, spurred a
reactive need to redefi ne the line and assert its priority
as the most distinguishing marker of poetry. Accordingly,
James Longenbach and others have argued for
discarding the term line breaks for the more accurate
fulfi llment , since a line is not “broken”; it simply ends
before another begins. Th e value placed on line integrity
requires that a line be “fulfi lled,” i.e., that it have
reason for being a piece of meaning, aff ect, and sound,
as opposed to a randomly sliced bit of chopped prose.
Similarly, a stanza (It. for “room”) needs to be organized
as a room of its own at the same time that it
contributes to the whole. For Hollander and others, a
verbal work must achieve the fi gurative level of metaphor
to be a poem.

Th ese aspects of poetry point more
clearly to the qualitative ends of verse craft: principles,
assumptions, rules, guidelines, etc., exist for the writing
of good poetry. When poetry was largely synonymous
with verse and verse meant metered lines , versifi cation
pertained mostly to descriptions of craft. Now that
boundaries between verse and prose have become less
distinct and poetry, for many, serves as a general term
for artful lang., discussions of versifi cation have necessarily
become more prescriptive, as they advance particular
views of what poetry is or should be.
 W imsatt; P. Fussell, P oetic Meter and Poetic Form ,
rev. ed. (); J. Hollander , Figure of Echo (),
and Rhyme’s Reason: A Guide to English Verse ();
Attridge, Rhythms ; Th e Line in Postmodern Poetry, ed.
R. J. Frank and H. M. Sayre (); G. T. Wright,
Shakespeare’s Metrical Art (); J. McCorkle, ed.,
Conversant Essays, Contemporary Poets on Poetry
(); T. Steele, Missing Measures: Modern Poetry
and the Revolt against Meter (); S. Cushman, Fictions
of Form in American Poetry (); Gasparov,
History; H. Gross, Sound and Form in Modern Poetry ,
d ed. (); Finch and Varnes; R. Abbott, “T. S.
Eliot’s Ghostly Footfalls: Th e Versifi cation of ‘Four
Quartets,” Cambridge Quarterly  (): –;
Radiant Lyre: Essays on Lyric Poetry , ed. D. Baker and
A. Townsend (); J. Longenbach, Th e Art of the
Poetic Line ().

The rhythm of a linguistic utterance is basically the sequence of syllable-related accent values (associated with pitch, duration and loudness values) resulting from the 'natural' pronunciation of a sentence or text by a competent speaker who takes into account the learned inherent word accents as well as syntax- and discourse-driven accents. All acquired top-down knowledge of lexicon, syntax, and prosody of the whole language goes into this pronunciation, but not any particular meter construct. In this 
%particularly relevant latter 
sense, rhythm is driven bottom-up by the wording of sentences. 

In particular uses of language (proverbs, slogans, poems, songs), the rhythm is over-regulated in the direction of a genuine meter. In silent reading of poems, a meter expectation based on acquired knowledge is usually already triggered by the visual perception of a strophic structure. 

%Moreover, German (or English) readers know from experience, for example, that where there is an end rhyme, there is also a meter. (Rhyme is, at least in German, a para-metrical phenomenon. Conversely, there is also meter without rhyme). 

When listening, the perception of an artificially (over)regulated meter is also and especially bottom-up in a relatively short time. Once a meter has been developed (be it top-down and visually, be it bottom-up in the process of silent reading or listening), it is built into the expectation, and it thus acquires the status of a top-down construct that guides (further) reading (on revocation).
Basically, therefore, a meter is primarily, though by no means exclusively and always, an artificial top down construct. Rhythm, on the other hand, is more bottom-up and arises all by itself from 'natural' prosody. 
%In your assignments of the 4 terms rhythm, meter, top down and bottom up, it goes back and forth in many places, even though it seems to me that you mostly share my understanding outlined above. There is still more and clearer consistency required.

C. O. Hartman
ACCENT In Eng., accent is the auditory prominence
perceived in one syllable as compared with others in
its vicinity. Accent and stress are often treated as synonymous,
though some literary scholars and linguists
distinguish the two terms according to a variety of
criteria. Disagreements persist about the source and
acoustical nature of syllabic prominence—loudness,
volume, *pitch, *duration, or some combination of
factors—but they are arguably of peripheral relevance
to the understanding of accent within Eng. poetics.
Th e phenomena of accent vary among langs. and
the poetics associated with them. Th e Eng. lexical
contrast between convict as noun and as verb has no
parallel in Fr. (Sp. resembles Eng. in this regard, while
Finnish resembles Fr.) For Fr. speakers, stress contours
are perceived on the level of the phrase or clause, and
learning Eng. entails acquiring the ability to hear contrastive
accent in words, just as a Japanese speaker
learning Eng. must acquire the distinction between
the liquids l and r . A consequence is that, while Fr.
*meters count only *syllables, Eng. meters conventionally
also govern the number and distribution of
accents.
In Eng. speech, accent operates in various ways on
scales from the word ( convict ) through the sentence.
As the units grow larger, accent becomes increasingly
available to choice and conscious use for rhetorical emphasis.
One step beyond the accents recorded in dicts.
is the diff erence between “Spanish teacher” as a compound
(a person who teaches Sp.) and as a phrase (a
teacher from Spain). Eng. phonology enjoins stronger
accent on “Spanish” in the compound and “teacher” in
the phrase

Readers are sensitive to a far wider range of rhythmic
phenomena in poetry than those that are encoded
within a metrical system. Th e nuanced stress patterns
of speech, though they are foregrounded in nonmetrical
or *free verse, do not disappear from the reader’s
awareness in metrical verse with its two-valued feature
of accent. Rather, the give and take between the claims
of meter and rhythm become a major source of auditory
richness. Syllables may be heard as stressed either
because of their prominence in speech or because of
their position within the metrical line.

Two-element *meters tend to maintain the stability
of the lines’ measure without as much rigidity in adherence
to the meter’s defi ning rules as single-element
meters require. Consequently, much of the richness of
variation in a two-element meter such as the accentualsyllabic
can be captured at least crudely by analysis of
substituted feet, metrical inversions, promoted stresses,
and similar concepts that build on the notion of the
*foot. Th is variety can be sketched or roughly diagrammed
by *scansion of the lines.
Particular meters in such a two-element system are
conventionally named by combining an adjectival form
of the name of the base foot (iambic, dactylic, trochaic,
etc.) with a noun made of a Lat. number word plus
“-meter”: trimeter, tetrameter, pentameter, hexameter,
and so on.

Meter is the *measure of sound patterning in verse,
occurring when a *rhythm is repeated throughout a
passage of lang. with such regularity that a base unit
(such as a *foot) becomes a norm and governs poetic
composition. Meter is an idealized pattern, a cultural
construct understood as artistic shaping of the sound
pattern of a lang. All langs. possess the makings of
metrical systems. Metrical verse works the basic properties
of a given lang. to a more highly regularized
level. When studying meters, one focuses on their
historical changes, on their cultural associations, and
on describing and analyzing specifi c meters shaped
by individual poets into metrical styles. As cultural
constructs, meters are a major part of verse design.
While design, like rhythm, is innate for humans desiring
a sense of order, designs are made, learned, and
passed on in a culture. Th ey are open to innovation
and transcend the linguistic material of which they
are made (Hollander; Cushman). As a regularized
organization of *sound, metrical design both uses
and pulls against the speech patterning of lang. Th e
ordinary rhythms of a lang. must rise to an unusual
degree of prominence to become a meter. As a result,
meter can heighten emotion and compete with sense.
Aristotle noticed that a too-heightened rhythm could
override sense and persuade, an eff ect Roman Jakobson
regarded as the basis of the *poetic function
(Sebeok). Julia Kristeva sees in this poetic function the
argument between the rhythmic (the feminine) and
the rational (the law, the masculine) dimensions of
lang. (Cook).
Cultures develop particular verse trads. based on
normative meters that are recognized tacitly as well
formed or not, indicating that the rules are made by
cultures and learned in the same way lang. competence
is acquired. For this reason, meters also change;
“rules” restrict what may count as metrical for a particular
time and place, i.e., what linguistic situations
in the verse may occur when exceptions to the norm
appear in a verse meter (see individual entries for specifi
c langs. and lit. hists., e.g., arabic prosody; celtic
prosody; china, poetry of ). Measurement of verse
in a given lang. may depend primarily on *quantity,
*accent (stress), *syllable, tone (*pitch), or *syntax.
One of these will be the dominant component of a
meter, and one or more of the others may aff ect it, but
full descriptions of the infl uence on metrical patterning
of secondary features, such as *rhyme and sound
(in all langs.; see Crystal), are still being developed by
linguists.
In a stress-based lang. like Eng., two levels of
stress—strong and weak—defi ne the normative pattern
that forms the idealized metrical base. Identifying
the meter of a poem or part of a poem is accomplished
by a process of marking stresses, called scanning , and
yields a *scansion. In actuality, the idealized pattern
is realized at three or four perceptual levels of stress.
Th e term scansion has been traditionally reserved for
marking the idealized pattern, but since the s,
theories using ling. have marked three or four levels
in order to develop descriptive and explanatory “rules”
(see below; see generative metrics, relative stress
principle ). Within these relative perceptual levels, the
basic pattern can be perceived because the adjacent
stresses remain weak or strong relative to each other
(Chatman; Halle and Keyser). Th e actual levels of
stress compose the rhythm of the passage and create
sound, meaning, and expressive qualities specifi c to a
poem. Th e idealized pattern gains fl exibility or rigidity
depending on “allowable” departures that have been
built up (and continue to be built up) as a trad. of metrical
composition by poets’ adding new variations on
the metrical base. Th e numbers and location of weak
and strong stresses that comprise a unit defi ne the type
of meter. New meters that are devised may enter the
metrical code of a literary trad. with suffi cient use by
poets and recognition by readers.
Four metrical categories are traditionally recognized
in Eng. poetry, named for the distinguishing factor that
establishes the unit of measure: accentual, accentualsyllabic
(also known as accentual isosyllabic), syllabic
(also known as isosyllabic), and quantitative (though
this category is controversial; see below). Th e name of
a metrical type (e.g., *ballad, *iambic *pentameter) refers
variously to the poetic trad. of that meter, to an entire
poem, to a section of a poem, or to the line pattern.
Meter inhabits a context, as is demonstrated by lines
that might be scanned as more than one meter if they
occurred in diff erent metrical contexts.
Th e concept of measuring verse into units, called
feet, and units into lines with a specifi ed number of
feet is an analytic one, originally imposed by the
Greeks on poetic compositions as a way of describing
the disciplining of rhythmic repetition into lines
of verse when verse was written down. (Gr. prosodists
were divided between the rhythmikoi , who measured
by rhythm, as in music, and the metrikoi , who measured
by foot.) Measuring meter in feet is known as
the classical approach to meter; it was imported into
Eng. during the Ren. and has prevailed as a guide to
verse composition and prosodic study as infl uenced by
Romance verse. Other approaches have been developed
in the th c., thanks to mod. ling., scientifi c methods
and goals of investigation, and the explosion of
nonmetrical poetry. Th e most important of these have
been systems grounded in generative metrics, linguistic

II. Debates About Meter . Disagreements over meter
tend to be contentious and entrenched, pitting the cl.
approach against mod. ling., and linguists themselves
divide over basic issues such as what is the motivation
for prominence assignment; whether meter involves
only measurable sound features of the foot or whether
meter cannot be separated from the rhythmic infl uence
of higher level systems and nontemporal sound
structures; whether musical theory applies to meter;
whether actual readers’ perceptions are relevant to
meter; and whether a universal theory of meter is possible
(see linguistics and poetics ).
At the opposite extreme from the cl. approach are
theories that admit only one type of meter in Eng. Some
theorists have asserted that meter in Eng. is trochaic,
citing the pronunciations of Germanic words and compounds,
which stress the onset syllable, whereas others
argue that Eng. is iambic, with line onset stresses
adjusted to iambs by postulating a silent uptake before
the stressed onset (Wallace and essays on this
debate in Baker). Latinate words, by contrast, prefer
an iambic rhythm, with the two heritages mixing
to comprise the two basic meters, as well as the
variety seen in iambic pentameter. In the iambic- only
view, *anapests are elided iambs, *dactyls are elided trochees,
and *spondees are iambs as their relative stress
assignments show. Debates over these issues indicate
that meter in mod. Eng. combines accentual and syllabic
features. From the oldest existing poetry in Eng.
to mod. free verse, units are built of stressed syllables
with a varying but always limited number of relatively
weaker syllables surrounding them. Th is character is
perhaps inevitable given the alternating stress pattern
of Eng. and the regularity of repetition that makes for
perception of meter.

III. Functions . Meter signals *genre, elicits the pleasures
of musicality in expectation and surprise, imitates
meaning in the content (see iconicity, mimesis ),
contributes to *tone (e.g., ironic, satiric, oracular, conversational),
and bears social and cultural meanings.
Th e fi rst three of these functions were much studied
by *New Criticism and *structuralism (essays in Sebeok
and in Chatman and Levin). Th e last two of these
functions have been most neglected despite their
analytic potential with respect to critical and cultural
studies (Hurley). Because the defi nitions and limits
of meters are preferences of a group or a time, what is
called a meter can change, and the theories and functions
of meter will also change over time.

\fi

==> 031_corpora_small.tex <==


\section{Manually Annotated Corpora}

With the goal of learning particularly rhythmic features, we found two previously annotated datasets of Modern English poetry. We annotate additional poems for English, and build an annotated dataset for the New High German language from scratch. 


\iffalse
For Better Meter
Wrong 262 Right 873
Train Len 698
Test Len 87
Val Len 88

For Better Real
Wrong 71 Right 1064 Comment 0
Train Len 851
Test Len 106
Val Len 107

For Better Real Meter
Wrong 49 Right 1084 Comment 0
Train Len 867
Test Len 108
Val Len 109

Prosodic Lit Lab Sample Meter
Wrong 173 Right 1564 Comment 0
Train Len 1251
Test Len 156
Val Len 157

EPG64 Meter
Wrong 114 Right 1098 Comment 0
Train Len 878
Test Len 110
Val Len 110
\fi 

\subsubsection{English Rhythm Gold Corpus}

The English corpus with manual annotation was collected from three sources: (1) The for-better-for-verse (FORB) collection\footnote{\url{https://github.com/manexagirrezabal/for_better_for_verse/tree/master/poems}} with around 1200 lines which was used by \newcite{agirrezabal-etal-2016-machine,agirrezabal2019comparison}. (2) The 1700 lines of poetry against which \texttt{prosodic}\footnote{\url{https://github.com/quadrismegistus/prosodic}} \cite{algee2014stanford} was evaluated (PROS), and finally (3) the 1200 lines in 64 English poems (EPG64) that were previously annotated for aesthetic emotions by \newcite{haider2020po}. The first two corpora were already annotated for syllable stress. EPG64 is annotated with the same guidelines as the following German corpus. FORB does not contain readily available foot boundaries, and in PROS foot boundaries are occasionally set after each syllable. Additionally, FORB makes use of a \texttt{<seg>} tag to indicate syllable boundaries, making it cumbersome to derive the position of a syllable in a word. It also contains two competing annotations, \texttt{<met>} and \texttt{<real>}.\footnote{\texttt{<met>} is the supposedly proper metrical annotation, while \texttt{<real>} is an annotation according to a more natural rhythm (with a tendency to accept inversions and stress clashes). We only choose \texttt{<real>} when \texttt{<met>} doesn't match the syllable count (ca. 200 cases).} 

\begin{table}
    \centering
    \begin{footnotesize}
    \begin{tabular}{lrrrr} 
        \toprule 
         & German & EPG64 & FORB & PROS \\ 
         \cmidrule(r){1-1}\cmidrule(rl){2-2}\cmidrule(l){3-3}\cmidrule(l){4-4}\cmidrule(l){5-5}
         \# correct lines & 3431 & 1098   & 1084 & 1564 \\
         \# faulty lines & 58 & 114      & 49 &  173 \\
%         \# train lines & - & 878       & 867 & 1251 \\
%         \# test lines & - & 110        & 108 & 156 \\
%         \# dev lines & - & 110         & 109 & 157 \\
         \bottomrule
    \end{tabular}
    \caption{Size of manually annotated corpora. Faulty lines denotes the number of lines where the automatic syllabification failed. Correct lines are used for experiments, since only there the annotation aligns.}
    \label{table:data_statistics}
    \end{footnotesize}
\end{table}


%The English corpus contains 64 poems of popular English writers. It
%was partly collected from Project Gutenberg with the GutenTag
%tool,\footnote{\url{https://gutentag.sdsu.edu/}} and, in addition,
%contains a number of hand selected poems from the modern period and
%represents a cross section of popular English poets. We took care to
%include a number of female authors, who would have been
%underrepresented in a uniform sample. Time stamps in the corpus are
%organized by the birth year of the author, as assigned in Project
%Gutenberg.


\subsubsection{German Rhythm Gold Corpus}

The small German corpus is fairly diverse, considering its size, and covers not only a wide range of different poem lengths and verse measures but also a number of influential German poets of both genders. \citet{haider2020po} previously annotated this corpus for aesthetic emotions. We annotate it for binary syllable prominence, foot boundaries, caesuras, and the main accents of a line. Besides the annotation of poetic features, every poem also has information on the author name, a title, the year of publication, and literature periods. We exclude two Middle High German poems by Walther von der Vogelweide and three poems in free rhythm (by Goethe) that do not allow for a metrical analysis, effectively amounting to 3.489 lines in 153 poems, spanning a time period from 1636 to 1936 CE. This yields a corpus that is somewhat representative for classical New High German poetry, while remaining manageable for manual annotation. 



==> 06_generating.tex <==
%\section{Style Transfer \& Emotion}

%\subsection{Metrical Paraphrasing}

%Pre tune a pre-trained BART model on three paraphrasing datasets.

%We take this vanilla model to classify its output by verse measure, and see if and how often the meter changes.

%We then condition BART during training on different verse measures.
\newpage 

\section{The Influence of Rhythm on Emotion Detection}

%\section{Prosodic Signal for Emotion Detection}
12 LAYER \\
BASE BERT VANILLA \\
MLP Regressor \\
R2: 0.4464949245868308 \\
R2 Sklearn: 0.2000439199024675 \\
Pearson: (0.6848554065063465, 3.349805046227404e-278) \\
Mean absolute error: 0.19071904874588153 \\

BASE VANILLA + ONEHOT Measure \\
MLP Regressor \\
R2: 0.46776318916353943 \\
R2 Sklearn: 0.14394190252721561 \\
Pearson: (0.6911729550454094, 2.122276506877456e-285) \\
Mean absolute error: 0.1837578758206275 \\

BASE HEADPROCESSOR \\
MLP Regressor \\
R2: 0.3849501218935461 \\
R2 Sklearn: -0.18685484399382002 \\
Pearson: (0.6283728847918004, 3.546783606409025e-221) \\
Mean absolute error: 0.19475225831684614 \\

BASE HEADPROCESSOR + ONEHOT Measure \\
MLP Regressor \\
R2: 0.38975262292798296 \\
R2 Sklearn: 0.025600834391313665 \\
Pearson: (0.6428975025853815, 1.0837593897634553e-234) \\
Mean absolute error: 0.19678825042000678 \\

Bert-Large Frozen + MLP (100 hidden layer): \\
Last 4 Layer:  \\
.61812 Bert Vanilla, R2: .213, mae .231
\\
.631 + FMeasure one-hot (55), R2: .271, mae .218 \\

Last 2 Layer: \\
.61759 Bert Vanilla, R2: .236, mae .225 \\
.62241 + FMeasure one-hot (55), R2: .284, mae .219 \\

6 Layer Fmeasure \\
R2: 0.4804207232473754 \\
R2 Sklearn: 0.23231607112177022 \\
Pearson: (0.7104869038887519, 1.313921709818356e-308) \\
Mean absolute error: 0.1812874046104333 \\

Vanilla 6 Layer: \\
R2: 0.49102615484751755 \\
R2 Sklearn: 0.29131760141237695 \\
Pearson: (0.7218940839682544, 3e-323) \\
Mean absolute error: 0.17874534320224372 \\

Vanllia 12 Layer \\
R2: 0.5084672655150366 \\
R2 Sklearn: 0.30140307868380956 \\
Pearson: (0.7238894170602813, 0.0) \\
Mean absolute error: 0.17398760222333726 \\

Measure 12 Layer \\
R2: 0.48761045985111795 \\
R2 Sklearn: 0.17257208527254642 \\
Pearson: (0.7101044942042687, 3.9503278276117475e-308) \\
Mean absolute error: 0.17927741779767647 \\

Short Measure 12 Layer \\
R2: 0.4617920569189805 \\
R2 Sklearn: 0.14514932654855672 \\
Pearson: (0.6878025635918931, 1.54885656145262e-281) \\
Mean absolute error: 0.18326839034730175 \\

==> 09_instructions.tex <==








\clearpage

\subsection{Hyperlinks}
Within-document and external hyperlinks are indicated with Dark Blue text, Color Hex \#000099.

\subsection{Citations}
Citations within the text appear in parentheses as~\citep{Gusfield:97} or, if the author's name appears in the text itself, as \citet{Gusfield:97}.
Append lowercase letters to the year in cases of ambiguities.  
Treat double authors as in~\citep{Aho:72}, but write as in~\citep{Chandra:81} when more than two authors are involved. Collapse multiple citations as in~\citep{Gusfield:97,Aho:72}. 

Refrain from using full citations as sentence constituents.
Instead of
\begin{quote}
  ``\citep{Gusfield:97} showed that ...''
\end{quote}
write
\begin{quote}
``\citet{Gusfield:97} showed that ...''
\end{quote}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \small\verb|\citep| & \small\verb|\cite| \\
\citealp{Gusfield:97} & \small\verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \small\verb|\citet| & \small\verb|\newcite| \\
\citeyearpar{Gusfield:97} & \small\verb|\citeyearpar| & \small\verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

\paragraph{\LaTeX-specific details:}
Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command {\small\verb|\citet|} (cite in text) to get ``author (year)'' citations as in \citet{Gusfield:97}.
You can use the command {\small\verb|\citep|} (cite in parentheses) to get ``(author, year)'' citations as in \citep{Gusfield:97}.
You can use the command {\small\verb|\citealp|} (alternative cite without  parentheses) to get ``author year'' citations (which is useful for  using citations within parentheses, as in \citealp{Gusfield:97}).


\subsection{References}
Gather the full set of references together under the heading \textbf{References}; place the section before any Appendices. 
Arrange the references alphabetically by first author, rather than by order of occurrence in the text.

Provide as complete a citation as possible, using a consistent format, such as the one for \emph{Computational Linguistics\/} or the one in the  \emph{Publication Manual of the American 
Psychological Association\/}~\citep{APA:83}.
Use full names for authors, not just initials.

Submissions should accurately reference prior and related work, including code and data.
If a piece of prior work appeared in multiple venues, the version that appeared in a refereed, archival venue should be referenced.
If multiple versions of a piece of prior work exist, the one used by the authors should be referenced.
Authors should not rely on automated citation indices to provide accurate references for prior and related work.

The following text cites various types of articles so that the references section of the present document will include them.
\begin{itemize}
\item Example article in journal: \citep{Ando2005}.
\item Example article in proceedings, with location: \citep{borschinger-johnson-2011-particle}.
\item Example article in proceedings, without location: \citep{andrew2007scalable}.
\item Example arxiv paper: \citep{rasooli-tetrault-2015}. 
\end{itemize}


\section{Translation of non-English Terms}

It is also advised to supplement non-English characters and terms with appropriate transliterations and/or translations since not all readers understand all such characters and terms.
Inline transliteration or translation can be represented in the order of:
\begin{center}
\begin{tabular}{c}
original-form \\
transliteration \\
``translation''
\end{tabular}
\end{center}
